3D Molecular Generation via Virtual Dynamics

Structure-based drug design, i.e., finding molecules with high affinities to the target protein pocket, is one of the most critical tasks in drug discovery. Traditional solutions, like virtual screening, require exhaustively searching on a large molecular database, which are inefficient and cannot return novel molecules beyond the database. The pocket-based 3D molecular generation model, i.e., directly generating a molecule with a 3D structure and binding position in the pocket, is a new promising way to address this issue. Herein, we propose VD-Gen, a novel pocket-based 3D molecular generation pipeline. VD-Gen consists of several carefully designed stages to generate fine-grained 3D molecules with binding positions in the pocket cavity end-to-end. Rather than directly generating or sampling atoms with 3D positions in the pocket like in early attempts, in VD-Gen, we first randomly initialize many virtual particles in the pocket; then iteratively move these virtual particles, making the distribution of virtual particles approximate the distribution of molecular atoms. After virtual particles are stabilized in 3D space, we extract a 3D molecule from them. Finally, we further refine atoms in the extracted molecule by iterative movement again, to get a high-quality 3D molecule, and predict a confidence score for it. Extensive experiment results on pocket-based molecular generation demonstrate that VD-Gen can generate novel 3D molecules to fill the target pocket cavity with high binding affinities, significantly outperforming previous baselines.

==> Figures/model_optim.tex <==
 \begin{figure*}[ht]%
 %\vspace{-0.1cm}
\includegraphics[width=1.0\linewidth]{Pictures/model_optim.pdf}%
\caption{Extending \texttt{VD-Gen} to molecular optimization.} \label{fig:model_optim}

\end{figure*}%

==> Figures/pocket_cavity.tex <==
 \begin{figure}[t]%
 %\vspace{-0.1cm}
 \centering
\includegraphics[width=0.3\linewidth]{Pictures/pocket_cavity.jpg}
\vspace{-10pt}
\caption{A case to show the detected pocket cavity.} \label{fig:pocket_cavity}
\vspace{-10pt}
\end{figure}%

==> Tables/denovo-main.tex <==

%这些表都存在一个问题就是没有值就补0
%有些值缺失太多感觉会是个问题
%ligan需要重新看看排除空的分子
%我们的模型也需要重新控制选择lddt不一样的分子
% \begin{table}[htbp]
%   \centering
%   \caption{Overall Results)}
%   \vspace{5pt}
%     \begin{tabular}{c|ccccc}
%     \toprule
%     Metric & Valid & Uni & QED($\uparrow$) & SA($\uparrow$) & LogP   \\
%     \midrule
%     GraphBP & 1.0 & 1.0 & 0.418 & 0.457 & 3.457 \\
%     LiGAN  & 0.986 & 0.949 & 0.442 & 0.609 & 0.105 \\
%     3DSBDD  & 0.956 & 0.954 & 0.503 & 0.610 & 1.151 \\
%     Pock2mol & 1.0 & 1.0 & 0.590 & 0.756 & 1.128 \\
%     target  & - & - & 0.411 & 0.673 & 0.691 \\
%     Our  & 1.0 & 0.973 & 0.495 & 0.603 & 0.424  \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:addlabel}
%   \vspace{-5pt}
% \end{table}




% \begin{table}[htbp]
%   \centering
%   \caption{Overall Results)}
%   \vspace{5pt}
%     % \begin{tabular}{c|cccccccc}
%     \begin{tabular}{p{0.18\columnwidth}|p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}}
%     \toprule
%     Metric & Vina($\downarrow$) & Higher Affi(\%$\uparrow$) & 3D sim($\uparrow$) & High sim(\%$\uparrow$) & 2D Div & PBSA($\downarrow$)  & Higher PBSA($\downarrow$) & PBSA Rank($\downarrow$) \\
%     \midrule
%     GraphBP  & -6.765 & 0.171 & 0.353 & 0.002 & 0.065 & -41.221 & 0 &  2.646 \\
%     LiGAN    & - & - & 0.356 & 0.011 & 0.037 & -12.472 & 0 & 2.091 \\
%     3DSBDD   & - & - & 0.365 & 0.015 &  0.144 & -24.789 & 0.001 & 2.171 \\
%     Pock2mol & - & - &  0.352 & 0.007 & 0.135 & -10.573 & 0 & 2.404\\
%     Our  & - & - & 0.414 & 0.116 & 0.226 & -48.090 &  0.043 & 1.162\\
%     GraphBP(UFF)  & -6.765 & 0.171 & 0.353 & 0.002 & 0.065 & -41.221 & 0 &  2.646 \\
%     LiGAN(UFF) & -4.219 & 0.018 & 0.361 & 0.013 & 0.044 & -14.863 & -0.001 & 2.373 \\
%     3DSBDD(UFF)   & -5.630 & 0.083 & 0.373 & 0.022 & 0.159 & -39.961 & 0.009 & 2.202 \\
%     Pock2mol(UFF) & -3.548 & 0.034 & 0.341 & 0.009 & 0.142 & -24.207 & 0.002 & 2.333\\
%     Our(UFF)  & -5.825 & 0.076 & 0.410 & 0.148 & 0.221 & -48.242 & 0.057 & 1.455\\
%     GraphBP(ReDock)  & -6.765 & 0.171 & 0.353 & 0.002 & 0.065 & -41.221 & 0 &  2.646 \\
%     LiGAN(ReDock) & -5.740 & 0.076 & 0.359 & 0.018 & 0.062 & -17.228 & 0.001 & 2.384 \\
%     3DSBDD(ReDock) & -7.550 & 0.260 & 0.373 & 0.021 & 0.144 & -38.748 & 0.005 & 2.030 \\
%     Pock2mol(ReDock) & -7.467 & 0.260 & 0.371 & 0.025 & 0.143 &  -29.571 & 0.009 & 2.171 \\
%     target  & -8.042 & - & - & - & - & - & -\\
%     Our(ReDock)  & -7.958 & 0.294 & 0.383 & 0.068 & 0.235 & -53.059 & 0.031 & 1.616\\
    
    
%     \bottomrule
%     \end{tabular}
%   \label{tab:addlabel}
%   \vspace{-5pt}
% \end{table}



==> Tables/molecular-optimization.tex <==

%这些表都存在一个问题就是没有值就补0
%有些值缺失太多感觉会是个问题
%ligan需要重新看看排除空的分子
%我们的模型也需要重新控制选择lddt不一样的分子
% \begin{table}[htbp]
%   \centering
%   \caption{Overall Results)}
%   \vspace{5pt}
%     \begin{tabular}{c|ccccc}
%     \toprule
%     Metric & Valid & Uni & QED($\uparrow$) & SA($\uparrow$) & LogP    \\
%     \midrule
%     DeepFrag & 1.0 & 1.0 & 0.430 & 0.686 & 1.154 \\
%     target  & - & - & 0.411 & 0.673 & 0.691 \\
%     Our  & 1.0 & 0.998 & 0.442 & 0.598 & 0.198  \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:addlabel}
%   \vspace{-5pt}
% \end{table}




% \begin{table}[htbp]
%   \centering
%   \caption{Overall Results)}
%   \vspace{5pt}
%     \begin{tabular}{p{0.18\columnwidth}|p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}}
%     \toprule
%     \toprule
%     Metric & Vina($\downarrow$) & High Affi(\%$\uparrow$) & 3D sim($\uparrow$) & High sim(\%$\uparrow$) & 2D Div & PBSA($\downarrow$)  & High PBSA($\downarrow$) & PBSA Rank($\downarrow$) \\
%     \midrule
%     DeepFrag  & -7.775 & 0.273 & 0.431 & 0.220 & 0.682 & -52.656 & 0.128 & 1.414 \\
%     target  & -8.042 & - & - & - & - & -51.335 & - & - \\
%     Our  & -6.208 & 0.052 & 0.781 & 0.947 & 0.431 & -51.933 & 0.374 & 1.333 \\
%     Our(UFF)  & -7.507 & 0.195 & 0.715 & 0.886 & 0.433 & -51.041 & 0.315 & 1.404 \\
%     Our(ReDock)  & -8.333 &0.423 & 0.491 &  0.391 & 0.435 & -50.7410 & 0.165 & 1.535 \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:addlabel}
%   \vspace{-5pt}
% \end{table}


